Hierarchical Interpolative Factorization for Self Green's Function in 3D Modified Poisson-Boltzmann Equations

The modified Poisson-Boltzmann (MPB) equations are often used to describe equilibrium particle distribution of ionic systems. In this paper, we propose a fast algorithm to solve MPB equations with the self Green's function as the self energy in three dimensions, where the solution of the self Green's function poses a computational bottleneck due to the need to solve a high-dimensional partial differential equation. Our algorithm combines the selected inversion with hierarchical interpolative factorization for the self Green's function by extending our previous result of two dimensions. This leads to an $O(N\log N)$ algorithm through the strategical utilization of locality and low-rank characteristics of the corresponding operators. Furthermore, the estimated $O(N)$ complexity is obtained by applying cubic edge skeletonization at each level for thorough dimensionality reduction. Extensive numerical results are performed to demonstrate the accuracy and efficiency of the proposed algorithm for problems in three dimensions.

==> figure/Level1_0.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{12.0cm}{!}{
\input{figure/fig-comp-modules/level1_0}
}


\end{minipage}
\caption{The DOFs in the first level.  The domain is partitioned into 16 blocks in the Level 1 and the dash lines show two of blocks in the decomposition. In this and following integral levels,  the interior points are marked in gray and the boundary points are marked in black. It's noted that the blocks share edge in practice to reduce the prefactor.}
\label{fig:lel1-0}
\end{figure}
